Bistatic Reflectivity and Micro-Doppler Signatures of Drones for Integrated Communication and Sensing

The integration of wireless communication and radar sensing is gaining the interest of researchers from wireless communication and radar societies. Sensing in Integrated Communication and Sensing (ICAS) systems differs from the traditional radar system in the configuration of transmitter-target-receiver, the operating frequency bands, and the transmitting waveform. It is necessary to understand how target electromagnetic signatures behave in this context. Therefore, this paper presents measurements and analysis of two important target signatures, reflectivity and micro-Doppler, for sensing in ICAS. These target signatures are measured in the state-of-the-art measurement system, Bistatische-Radar-Messeinrichtung (BiRa).

==> Makefile <==
BUILD_DIR=build
SHELL=/bin/sh
NAME=paper

default: full

.PHONY: clean
clean:
	rm -f arxiv.zip
	@ if [ -h $(BUILD_DIR) ] ; then \
		rm -rf `readlink $(BUILD_DIR)` ;\
		rm $(BUILD_DIR) ;\
	else \
		rm -rf $(BUILD_DIR) ;\
	fi

$(BUILD_DIR):
	@ if [ -h $(BUILD_DIR) ] ; then rm $(BUILD_DIR) ; fi
	ln -s `mktemp -d /tmp/$(NAME)-build.XXXXXXXX` $(BUILD_DIR)
	chmod 700 `readlink $(BUILD_DIR)`

.PHONY: full
full: $(NAME).tex $(BUILD_DIR)
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<
	BIBINPUTS="$(BUILD_DIR):" TEXMFOUTPUT="$(BUILD_DIR):" bibtex $(BUILD_DIR)/$(NAME)
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<

.PHONY: quick
quick: $(NAME).tex $(BUILD_DIR)/$(NAME).aux
	pdflatex -interaction nonstopmode -output-directory $(BUILD_DIR) $<

arxiv.zip: $(NAME).tex $(BUILD_DIR)/ Figures/
	cp -a $(BUILD_DIR)/$(NAME).bbl .
	zip -r arxiv.zip $(NAME).tex $(NAME).bbl orcidlink.sty Figures/
	rm $(NAME).bbl

